Convexity of Energy-Like Functions: Theoretical Results and Applications to Power System Operations

Power systems are undergoing unprecedented transformations with the incorporation of larger amounts of renewable energy sources, distributed generation and demand response. All these changes, while potentially making power grids more responsive, efficient and resilient, also pose significant implementation challenges. In particular, operating the new power grid will require new tools and algorithms capable of predicting if the current state of the system is operationally safe. In this paper we study and generalize the so-called energy function as a tool to design algorithms to test if a high-voltage power transmission system is within the allowed operational limits. In the past the energy function technique was utilized primarily to access the power system transient stability. In this manuscript, we take a new look at energy functions and focus on an aspect that has previously received little attention: Convexity. We characterize the domain of voltage magnitudes and phases within which the energy function is convex. We show that the domain of the energy function convexity is sufficiently large to include most operationally relevant and practically interesting cases. We show how the energy function convexity can be used to analyze power flow equations, e.g. to certify solution uniqueness or non-existence within the domain of convexity. This and other useful features of the generalized energy function are described and illustrated on IEEE 14 and 118 bus models.

==> IEEEtran/README <==

September 17, 2014


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8a has a number of significant changes over the v1.8 release.
For a full list of changes, please read the file changelog.txt. The most
notable changes include:


 1) Extensive rework of the compsoc mode to comply with the latest standards
    of the IEEE Computer Society.

 2) Fixed abstract, index terms and diamond line for compsoc technotes.

 3) New \IEEEraisesectionheading{} command to provide for the special
    raised first section heading of Computer Society journal papers.

 4) Internal code improvements for page setup and command argument
    processing.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_compsoc.tex, bare_jrnl_transmag.tex
***************************************************************************


==> Pflow.tex <==
%!TEX root=ConvexEnergyFunction.tex


%This corollary, although a simple consequence of our earlier results, has a powerful implication: We can solve the power flow equations (within reasonable operational constraints one would expect to hold in practice). Since the optimization problem inherits the structure of the power network, one can likely design distributed algorithms to solve the resulting optimization problems using techniques like ADMM \cite{boyd2011distributed}. We will investigate this in future work.

%Numerically, we have validated this technique on simple power system models that are testcases for the MATPOWER \cite{zimmerman2011matpower} software. In a small number of cases, it is able to find solutions when the standard MATPOWER AC solver cannot and in all cases, it is significantly more accurate than the DC solver. However, further work is needed to characterize exactly the regimes in which this approach will give accurate results.

\begin{comment}
\input{Duality.tex}
We present numerical results applying this method to the 6 bus network shipped with MATPOWER \cite{zimmerman2011matpower} (named ``case6ww''). We modify this network to have $0$ resistance and ignore shunt impedances etc, to get a network with purely inductive transmission lines. The network has 3 \PV and 3 \PQ buses. We investigate the following question:\\
Our convexity results require the reactive power demand to grow with voltage. If we make this approximation even though it is incorrect, do we get approximate but reliable solutions to the power flow equations? We investigate this by starting with the model with the given real and reactive power demands (for which a solution to the power flow equations exists and can be found by the default MATPOWER AC power flow solver). We then increase all the loads by a constant factor $\beta$. For a grid of values of $\beta \in [1,1.3]$, we solve the power flow equations using the default MATPOWER AC solver, the MATPOWER DC solver and a convex approach based on our results using an interior point mehtod (OPTI \cite{OPTI} MATLAB interface to IPOPT \cite{wachter2006implementation}). We compute the $\ell_2$ error in the power flow equations (normalized by the $\ell_2$ norm of $P$,$Q$) in the solution found by the three approaches as a function of $\beta$ and plot the results in figure \ref{fig:ConvexityPF}.

The results from figure \ref{fig:ConvexityPF} show that at small load scaling factors (upto $1.06$), the MATPOWER AC solver does well and is able to find accurate solutions. In this regime, our solver is slightly less accurate but much more accurate than the DC approximation. On increasing the loading further, the MATPOWER solver fails completely and gives highly inaccurate solutions. Our solver degrades more gracefully and is still able to find reasonably accurate solutions. It remains more accurate than both the DC and AC solver for all loading factors above, but the three solvers converge at very high loading factors. This shows that our approach, although requiring a potentially artificial assumption of reactive demand dependence on voltage, can find reasonably accurate solutions when in cases where traditional solvers (AC and DC) fail or are inaccurate. In fact, in practice the assumption of constant $P$ and $Q$ is an approximation and reactive power dependence of the form $Q_i\br{V_i}\propto V_I^\alpha$ with $\alpha \in [1.3,1.6]$ is quite common, so our approximation may be even more accurate than the results presented here.

\begin{figure}
        \centering
                \includegraphics[width=.9\columnwidth]{PFResults.pdf}
                \caption{Solving power flow equations: Comparison of three approaches}~\label{fig:ConvexityPF}
\end{figure}%
\section{Other Applications}\label{sec:GenApp}

In this section we briefly mention other possible applications of the energy function convexity results.

\subsection{Convex AC Optimum Power Flow}
%The basic idea is to view the energy function as being parameterized by the active and reactive power injections $P_i,Q_i$.
Let $P,Q$ denote the vectors of active and reactive power injections and we denote the energy function parameterized by these as $U\br{\rho,\theta;P,Q}$. Further, define a modified energy function that blows up outside the domain of convexity $\br{\rho,\theta}\in\C$.
%Let us consider the energy function dependence of $P$ and $Q$ -- injections/consumptions at the nodes and also define it auxiliary version pushed to be infinite outside of the domain of the energy function convexity (over $\rho$ and $\theta$)
\[\tilde{U}\br{\rho,\theta;P,Q} = \begin{cases}E\br{\rho,\theta|P,Q} & \text{ if} \br{\rho,\theta}\in\mathrm{int}\br{\C}(P,Q) \\ \infty & \text{otherwise} \end{cases}\]
Then formulate and solve the following new optimization problem
\[\min_{\br{\rho,\theta}\in S,P,Q} \lambda c(P,Q)+\tilde{U}\br{\rho,\theta;P,Q}\]
where $c\br{P,Q}$ is an exogenously given  cost on the injection/consumption and $S$ is a set specifying operational constraints on $\br{\rho,\theta}$ to be contained within $\mathrm{int}\br{\C}$. If we optimize with respect to $\br{\rho,\theta}$ keeping $P,Q$ fixed, we recover the active and reactive power balance equations (assuming a solution exists within $S$). Further, by choosing $\lambda$ sufficiently large, one can guarantee that the optimization with respect to $P,Q$ is not affected by the second term except to ensure that the active and reactive power balance equations are satisfied.

Observe that we have just formulated the AC Optimum Power Flow problem in terms of the energy function. As stated this optimization is not jointly convex in $\br{\rho,\theta,P,Q}$, however, one can additionally exploit ideas from the duality theory to reformulate it as a jointly convex optimization problem. For the simple case where voltage magnitudes are held fixed at all buses, related covexification strategy, based on the dual optimization formulation of PF problem introduced in \cite{12BV}, was discussed in \cite{bent2013synchronization}.

\subsection{Convex Model Predictive Control (MPC)}

The convexity results can also be used to obtain a convex formulation of model predictive control scheme for frequency and voltage regulation. Consider an optimal control problem that seeks to adjust active and reactive power injections at generators and loads in order to minimize frequency deviations while also maintaining operational constraints on voltage magnitudes and phases (for example see \cite{14AHa,14AHb}). The dynamical system under consideration here can be modeled by the DAE model given by \eqref{eq:swing} and \eqref{eq:PQReactive}. After discretizing time, one can enforce the dynamical constraints implicitly in the same way as discussed in the previous subsection. Again, using ideas from duality, the MPC optimization problem can be recast as a tractable convex optimization problem. Moreover, the resulting convex optimization will inherit the separable structure of the network and hence can be potentially solved in a distributed manner using algorithms like ADMM \cite{boyd2011distributed}. In future work, we will explore building on recent attempts to explore distributed optimization algorithms for power flow problems \cite{zhang2012optimal,zhao2013power,13SBC,Dall2013,Zampieri13c,magnusson2014distributed,peng2014distributed,Erseghe2014}, in order to get efficient distributed algorithms for our convex formulations of power flow and related problems.
%{\color{red} ... refs to recent ADMM applications in power systems may be excessive  ... may remove or shorten it later}

\subsection{Instantons}

As the penetration of intermittent sources of energy in the grid increases (through increased adoption of renewable generation like wind and Photovoltaics), an important problem is to characterize likely configurations of uncertain generation that would cause violation of operational constraints on voltage magnitudes and phases. This problem was studied using the DC power flow approximation in \cite{11CSPB,11CPS,12BS} where the problem was shown to be tractable through reduction to a small number of convex optimizations. The failure may be defined as line overload or nodal voltage leaving its safe range. More concretely, for overload on a line $(i,j)\in\E$, one would like to solve the following optimization problem:
\begin{eqnarray}
\max_w {\cal P}(w) \mbox{ s.t. }
\Biggl\{\begin{array}{c}
\mbox{PF Eqs. have a solution}\\
\mbox{line flow over $(i,j)$}\\
\mbox{is at the threshold}
\end{array}\Biggr.
\label{instanton}
\end{eqnarray}
where $w$ is the vector of uncertain generation and ${\cal P}(w)$ is its probability density. As stated,  the optimization \eqref{instanton} is not convex. However, as discussed in the previous sections, we can recast the power flow solution as the solution to a convex optimization of the energy function over voltages and phases. One can then generalizing the method of \cite{bent2013synchronization} (using the dual problem and restating \eqref{instanton} as single stage optimization over wind, voltage magnitudes and phases) one can derive a fully convex equivalent of the AC instanton problem \eqref{instanton}). Further details on this convex AC-instanton method will be pursued in future work.

\end{comment}

==> ReducedConvexity.tex <==
%!TEX root=ConvexEnergyFunction.tex

\section{Reduced Convexity}\label{sec:ReducedConvexity}
In section \ref{sec:Energy}, we examined various conditions under which the joint energy function $E\br{\rho,\theta}$ is jointly convex in $\br{\rho,\theta}$. However, as the numerical results (section \ref{sec:Num})indicate), these results are conservative and convexity of  $E\br{\rho,\theta}$ is only sufficient but not necessary for convexity of $E\br{\opt{\rho}\br{\theta},\theta}$. In this section, we examine the convexity of $E\br{\opt{\rho},\theta}$ directly. However, it will be convenient for us to work directly with the voltage variables $V$ rather than their logarithms $\rho$, so we will state our results in terms of  $E\br{V,\theta}$ and $E\br{\opt{V}\br{\theta},\theta}$.

\subsection{A Variational Representation for the Reduced Energy Function}

In this section, we develop a variational representation for the reduced energy function. As a simple corollary, we can also define a convex optimization problem that finds the solutions to the reactive power equations (the voltage magnitudes) given the voltage phases and a simple condition for uniqueness of the solution for voltage magnitudes within a given domain.


Before we proceed, we define some notation. Let $M\in\R^{n\times n}$ be such that
\begin{align}
M_{ij}=\frac{B_{ij}}{\sum_{j\neq i} B_{ij}}\label{eq:Mdef}
\end{align}
Let $M_{\Lo}$ be the $|\Lo|\times|\Lo|$ submatrix with row and column indices in $\Lo$. and $M_{\G}$ denote the $|\Lo|\times|\G|$submatrix with row indices indices in $\Lo$ and column indices in $\G$. Further, we define the normalized reactive power consumptions by
\begin{align}
\tilde{Q}_{i}=\frac{Q_{i}}{\sum_{j\neq i} B_{ij}}\label{eq:Qdef}
\end{align}
Further, we will assume that $Q_i>0$ at all \PQ~nodes, that is, we require that all \PQ~nodes consume reactive power. The more general case can also be dealt with, but we will focus on this case for now as the results are slightly simpler.

\begin{thm}\label{thm:RedCon}
Suppose that each load is connected to at least one generator. The reduced energy function can be expressed as follows:
\begin{align}
&\Et\br{\theta}  =\nonumber\\
&\min_{V_{\Lo}}  \sum_{i\in\Lo}  Q_i\logb{V_i}-\frac{1}{2}\sum_{\substack{i\in\Lo\\j\in\G}}B_{ij}V_i\Vset_j\cos\br{\theta_i-\theta_j}-\frac{1}{2}\sum_{i,j\in\G}B_{ij}\Vset_i\Vset_j\cos\br{\theta_i-\theta_j}  \label{eq:RedEnergy}\\
& \text{Subject to }  \nonumber \\
& \br{\sum_{j\neq i}B_{ij}}V_i^2-V_i\br{\sum_{j\neq i} B_{ij}V_j\cos\br{\theta_i-\theta_j}}+Q_i \leq 0 \quad\forall i\in\Lo\label{eq:SolveQuad}\\
& V_i=\Vset_i \quad \forall i \in \G \label{eq:ConstEq}\\
& V_i > \frac{2Q_i}{\sum_{j\in\G} B_{ij}\Vset_j\cos\br{\theta_i-\theta_j}}\forall i \in \Lo\label{eq:ConstEqTwo}
\end{align}
as long as the above optimization problem is feasible and $|\theta_i-\theta_j|\leq \frac{\pi}{2}$ for all $(i,j)\in\E$.
\end{thm}
\begin{proof}
We first show that the domain is compact. For $i\in\G$, $V_i$ is fixed by an equality constraint. Thus, each $V_i,i\in\Lo$ is bounded below by $0$ and above by lemma \ref{lem:BoundV}. Thus, the domain is compact and the optimization problem must have a finite minimum that is attained, if the problem is feasible.

Further, the objective is decreasing in $V_i$ for each $i\in\Lo$. Indeed, differentiating the objective with respect to $V_i$, we get
\[\frac{Q_i}{V_i}-\frac{1}{2}\sum_{j\in\G}B_{ij}\Vset_j\cos\br{\theta_i-\theta_j}\]
which is smaller than $0$ (using \eqref{eq:ConstEqTwo}). Thus, the objective is decreasing in $V_i$.  Also, if constraint \eqref{eq:ConstEqTwo} is satisfied for some value $V_i$, it is satisfied for all larger values.

We will now argue that constraint \eqref{eq:SolveQuad} must be tight at the optimum. The key observation is that for a given $i$, constraint $i$ is tight at two values of $V_i$ (roots of the quadratic equation) with the inequality being satisfied strictly at all intermediate values. We will argue that at the optimum, the constraint must be tight with $V_i$ being equal to the larger root. Suppose that this is not the case, that is let $\opt{V}$ be a (locally) optimal solution with constraint \eqref{eq:SolveQuad} not being tight at the optimum for some $i\in\Lo$. Then, one can increase $\opt{V}_i$ infinitesimally and reduce the objective while maintaining feasibility with respect to all the other constraints (since the other constraints are all satisfied more easily as $\opt{V}_i$ increases). This is a contradiction to $\opt{V}$ being a locally optimal solution.

Finally, it is easy to see that \eqref{eq:SolveQuad} with inequality replaced by equality simply reduces to the reactive power flow equations. Now, using lemma \ref{lem:RedFun}, the objective is equal to the reduced energy function at the optimum.
\end{proof}
\begin{remark}
The above representation gives us a way of computing voltage magnitudes (at \PQ buses) that solve the the reactive power equations given voltage phases, as long as the problem is feasible. Although this problem is nonconvex, as long as it is feasible, \emph{any} locally optimal solution is a solution to the reactive power equations. Below, we show that this can in fact be done via \emph{convex optimization}.
\end{remark}

\begin{corollary}
Let $c_i>0,i\in\Lo$ be an arbitrary set of positive numbers. A solution to the reactive power flow equations can always be found by solving the following convex optimization problem
\begin{align}
&\min_{\zeta_{\Lo}}  -\sum_{i\in\Lo}  c_i\zeta_i \label{eqc:RedEnergy}\\
& \text{Subject to }  \nonumber \\
& \br{\sum_{j\neq i}B_{ij}}\zeta_i-\br{\sum_{j\neq i} B_{ij}\sqrt{\zeta_i\zeta_j}\cos\br{\theta_i-\theta_j}}+Q_i \leq 0 \quad\forall i\in\Lo\label{eqc:SolveQuad}\\
& \zeta_i=\Vset_i^2 \quad \forall i \in \G \label{eqc:ConstEq}
\end{align}
as long as the above optimization problem is feasible and $|\theta_i-\theta_j|\leq \frac{\pi}{2}$ for all $(i,j)\in\E$ and setting $V_i=\zeta_i^2$. Further, by choosing all possible $c_i>0$, one can find the set of all solutions that are not dominated by any other (that is, all solutions such that no other solution to the reactive power flow equations has equal or higher voltage magnitudes at all \PQ buses).
\end{corollary}
\begin{proof}
The objective and constraints are easily seen to be convex in $\zeta_\Lo$. Further, the objective is strictly decreasing in $\zeta_i$ for each $i$. Hence, by the same argument as the previous theorem, any optimal solution must satisfy \eqref{eqc:SolveQuad} with equality (assuming the problem is feasible) at an optimal solution. Thus, any optimal solution must be a solution to the reactive power flow equations.

Further, this is a vector-convex optimization problem (see \cite{boyd2009convex} section 4.7). Thus, any vector $\opt{\zeta}_{\Lo}$ such that there is no $\zeta_{\Lo}\neq \opt{\zeta}_{\Lo}$ in the feasible set such that $\opt{\zeta}_{\Lo}\leq \zeta_{\Lo}$ is the solution to \eqref{eqc:RedEnergy} for some choice of $c_i>0$. This completes the proof. \end{proof}

\begin{remark}
Also note that these theorems did  not require the assumption that $Q_i>0$ but the results on convexity of the reduced energy function will.
\end{remark}

\subsection{Convexity of the Reduced Energy Function}

The representation from theorem \ref{thm:RedCon} shows that the reduced energy function is the solution to an optimization problem with an objective that is convex in $\theta$ and a convex constraint set on $\theta$. However, the objective and constraints are not convex in $V_i$ and hence we are unable to say anything about the convexity of the reduced energy function. In the following theorem, under additional assumptions, we show that the above optimization problem can be rewritten to show that the reduced energy function is convex. We will require a condition on the impedances and reactive power demands in order to get convexity. The least conservative way to state this condition is in terms of the solution to an optimization problem, which we define below:

\begin{align}
\overline{V_i}\br{B,Q}& =\max_{V_{\Lo}} V_i \label{eq:Bound}\\
&\text{Subject to }\nonumber \\
& \br{\sum_{j\neq i}B_{ij}}V_i^2-\sum_{j\neq i} B_{ij}V_iV_j+Q_i \leq 0 \quad\forall i\in\Lo \nonumber\\
& V_i=\Vset_i \quad \forall i \in \G \nonumber
\end{align}
This optimization problem can be solved as a convex optimization problem in the transformed variables $\zeta_i=V_i^2$.
\newcommand{\Vd}{\zeta}
\begin{thm}
Choose any $\Vpow \in (0,1)$. Let $c_{ij}>0$ be a set of positive numbers such that $Q_i=\sum_{j\neq i} c_{ij}B_{ij}$ for each $i\in\Lo$. Suppose that
\begin{align}
\overline{V_i}\br{B,Q}\leq\sqrt{\frac{1+\Vpow}{1-\Vpow}}\sqrt{\tilde{Q}_i} \quad\forall i \in \Lo\label{eq:ConvCondRed}
\end{align}
The reduced energy function can be expressed as
\begin{align}
&\Et\br{\theta}  =\nonumber\\
&\min_{\Vd_{\Lo}}  \sum_{i\in\Lo} \Vpow Q_i\logb{\Vd_i}-\frac{1}{2}\sum_{\substack{i\in\Lo\\j\in\G}}B_{ij}{\Vd_i}^{\Vpow}\Vset_j\cos\br{\theta_i-\theta_j}-\frac{1}{2}\sum_{i,j\in\G}B_{ij}\Vset_i\Vset_j\cos\br{\theta_i-\theta_j}  \label{eq2:RedEnergy}\\
& \text{Subject to }  \nonumber \\
& \br{\sum_{j\neq i}B_{ij}}\zeta_i^\beta+Q_i\zeta_i^{-\beta}\leq \sum_{j\neq i} B_{ij}\zeta_j^\beta\cos\br{\theta_i-\theta_j}  \quad \forall i\in\Lo\label{eq2:SolveQuad}\\
& \Vd_i={\Vset_i}^{\frac{1}{\Vpow}} \quad \forall i \in \G \label{eq2:ConstEq}\\
& {\Vd_i}^{\Vpow} >  \frac{2Q_i}{\sum_{j\in\G} B_{ij}\Vset_j\cos\br{\theta_i-\theta_j}}\quad\forall i \in \Lo\label{eq2:ConstEqTwo}\\
& \cos\br{\theta_i-\theta_j} \geq  \frac{c_{ij}}{\Vd^\Vpow}+\sqrt{\powb{\frac{c_{ij}}{\Vd^\Vpow}}{2}+\Vpow}\quad\forall i \in \Lo \label{eq2:ConstEqThree}
\end{align}
if the above optimization problem is feasible. Further, $\Et\br{\theta}$ is convex over the domain
\[\left\{\theta:|\theta_i-\theta_j|\leq\arccos\br{\sqrt{\Vpow}}\forall (i,j)\in\E,i,j\in\Lo,|\theta_i-\theta_j|\leq\arccos\br{\alpha}\forall\,(i,j)\in\E\right\}\]
\end{thm}
\begin{proof}
This problem is exactly equivalent to \eqref{eq:RedEnergy} with $\Vd_i=V_i^{\frac{1}{\Vpow}}$, except for the additional constraint \eqref{eq2:ConstEqThree}. Further, if this additional constraint is satisfied for some $\zeta_{\Lo}$, it is also satisfied for all larger $\zeta_{\Lo}$. Thus, the proof from theorem \label{thm:RedCon} is still valid and the above optimization problem, if feasible, attains its optimum and the constraint \eqref{eq2:SolveQuad} is tight at the optimum.
Now, on the given domain, it is easy to see that constraints  \eqref{eq2:ConstEq},\eqref{eq2:ConstEqTwo},\eqref{eq2:ConstEqThree} are all convex constraints in $\br{\rho_{\Lo},\theta}$ by lemma \ref{lem:Vcos}.

The last term in the objective is convex in $\theta$ and independent of $\zeta$.  The other terms can be rewritten as:
\[\sum_{i\in\Lo} \frac{1}{2}\sum_{j\in\G} B_{ij}\br{2\beta c_{ij}\logb{\zeta_i}-\zeta_i^\Vpow \cos\br{\theta_i-\theta_j}}\]
Each term in the above sum jointly convex in $\br{\rho_{\Lo},\theta}$ as long as constraint \eqref{eq2:ConstEqThree} is satisfied (by lemma \ref{lem:Vcos}).

Thus, the only thing remaining is the constraint \eqref{eq2:SolveQuad}. By lemma \ref{lem:radcos}, the RHS is concave in $\br{\rho_{\Lo},\theta}$ as long as
\begin{align}
\zeta_i^\Vpow  \leq \sqrt{\tilde{Q}_i}\sqrt{\frac{1+\Vpow}{1-\Vpow}}\label{eqthm:Red}
\end{align}
With $V_i=\powb{\zeta_i}{\frac{1}{\Vpow}}$, the constraint set defining the optimization problem \eqref{eq:Bound} is a relaxation of the constraints imposed in this problem, and hence  $\overline{V_i}\br{B,Q}$ is an upper bound on $\zeta_i^\beta$ for any $\zeta_{\Lo}$ in the feasible set. Hence, the constraint \eqref{eq2:SolveQuad} is convex as well.

Thus, the optimization problem is jointly convex in $\br{\zeta_{\Lo},\theta}$ and hence minimizing with respect to $\zeta_{\Lo}$ over the jointly convex domain produces a convex function of $\theta$. Hence the theorem.
\end{proof}

\begin{remark}
We tested the condition \eqref{eq:ConvCondRed} for some test networks in MATPOWER and found that for most cases, one can choose $\beta$ to satisfy \eqref{eq:ConvCondRed} such that $\arccos\br{\sqrt{\beta}}=10-20\deg$. This is a fairly stringent requirement and indicates that our analysis can be improved, although it is encouraging that the condition covers a non-trivial set of phases. The other set of constraints are typically satisfied under normal operating conditions, so the main source of conservatism in the convexity region estimate is \eqref{eq:ConvCondRed}, which in turn comes from requiring convexity of the LHS of \eqref{eq2:SolveQuad}. Thus, if we can deal with this more precisely (for example by using a convex relaxation and arguing tightness), we might be able to improve the estimates of convexity.
\end{remark} 
